Data Processing for Offline Evaluation in Recommender Systems: a Survey

Offline evaluation is the dominant experimental paradigm in recommender systems research, enabling reproducible and cost-effective comparisons on historical interaction data. Yet, while considerable attention has been devoted to recommendation models and evaluation methodologies, the data processing decisions that precede model training have received less scrutiny. These decisions determine the information available to recommendation algorithms and can affect the comparability and reproducibility of experimental results. This survey provides a systematic, cross-domain characterisation of data processing practices for the offline evaluation of recommender systems. We examine the data-centric pipeline, from dataset selection and interaction representation to data preparation, multimodal feature extraction, and train-validation-test splitting. Our analysis spans recommendation paradigms, including collaborative, sequential, session-based, graph-based, knowledge-aware, context-aware, multimodal, federated, cross-domain, contrastive-learning, and LLM-based recommendation. Beyond reviewing existing practices, we introduce a unified framework and taxonomy for describing data transformations and feature-extraction strategies, distinguishing data preparation from the extraction of representations from multimodal side information. Our empirical analysis reveals a landscape dominated by a narrow set of dataset-level transformations, particularly support-driven filtering, while representation-dependent transformations remain less common. We further identify substantial heterogeneity in how auxiliary information is prepared and represented, as well as inconsistencies in the specification of data splitting protocols, where similar labels may conceal different experimental conditions.

==> NOWFnT-data.tex <==
\newcommand\nowfnt@publicationaddress
 {%
  \textit{Published, sold and distributed by:}\\
  now Publishers Inc.\\
  PO Box 1024\\
  Hanover, MA 02339\\
  United States\\
  Tel.\ +1-781-985-4510\\
  www.nowpublishers.com\\
  sales@nowpublishers.com%
  \par
  \textit{Outside North America:}\\
  now Publishers Inc.\\
  PO Box 179\\
  2600 AD Delft\\
  The Netherlands\\
  Tel.\ +31-6-51115274
 }

\newcommand\nowfnt@legalrightstext
 {%
  All rights reserved. No part of this publication may be
  reproduced, stored in a retrieval system, or transmitted in any form or by any means, mechanical, photocopying, recording or otherwise, without prior written permission of the publishers.
  \par
  Photocopying. In the USA: This journal is registered at the Copyright  Clearance Center, Inc., 222 Rosewood Drive, Danvers, MA 01923.  Authorization to photocopy items for
  internal or personal use, or the internal or personal use of specific  clients, is granted by now Publishers Inc for users registered with the Copyright Clearance Center (CCC).
  The `services' for users can be found on the internet at:
  www.copyright.com
  \par
  For those organizations that have been granted a photocopy license, a separate system of payment has been arranged. Authorization does not extend to other kinds of copying, such as that for general distribution, for advertising or promotional purposes, for creating new collective works, or for resale.  In the rest of the world:
  Permission to photocopy must be obtained from the copyright
  owner. Please apply to now Publishers Inc., PO Box 1024, Hanover, MA 02339, USA; Tel. +1 781 871 0245; www.nowpublishers.com; sales@nowpublishers.com
  \par
  now Publishers Inc. has an exclusive license to publish this
  material worldwide. Permission to use this content must be obtained from the copyright license holder. Please apply to now Publishers, PO Box 179, 2600
  AD Delft, The Netherlands, www.nowpublishers.com; e-mail:
  sales@nowpublishers.com}

\newcommand\nowfnt@printedoninfotext
 {%
  {%
   %
  }%
 }

\newcommand\nowfnt@howtocitetext
 {%
  The preferred citation for this publication is\par
  {%
   \raggedright
   \useissuedata{copyrightowner}.
   \emph{\nowfnt@articletitle}.
   \printjournaltitleprefix \usejournaldata{title}, vol.~\useissuedata{volume}, no.~\useissuedata{issue}, pp.~\useissuedata{firstpage}--\useissuedata{lastpage},
   \useissuedata{pubyear}.%
  }%
 }


\newcommand\nowfnt@copyrightlinetext
 {%
  ISBN: \useissuedata{isbn}\\
  \copyright\ \useissuedata{copyrightyear} \useissuedata{copyrightowner}}

\newcommand\nowfnt@NOWcopyrightlinetext  %for wrapper
  {%
  ISBN: \useissuedata{isbn}\\
  \copyright\ \useissuedata{copyrightyear} Now Publishers Inc}

\newcommand\nowfnt@sourceintro{%
 The content of the book was originally published in  }

\newcommand\nowfnt@sourcepunct{.}

\newcommand\nowfnt@prohibitiontext{This article may be used only for the purpose of research, teaching, and/or private study. Commercial use or systematic downloading (by robots or other automatic processes) is prohibited without explicit Publisher approval.}

\newcommand\nowfntstandardcitation{\nowfnt@authorlist@toc\ (\nowfnt@issuepubyear), \enquote{\nowfnt@articletitle}, \nowfnt@journaltitle: Vol. \nowfnt@issuevolume, No. \nowfnt@issueissue, pp \nowfnt@issuefirstpage--\nowfnt@issuelastpage. DOI: \nowfnt@issuedoi.}

%Title for the series pages.
\newcommand\nowfnt@seriespagetitle{\section*{Other titles in \nowfnt@journaltitle}}

==> figures/datasets_frequency.tex <==
\definecolor{airforceblue}{rgb}{0.36, 0.54, 0.66}

\definecolor{pallidyellow}{HTML}{fee08b}

\begin{figure}[!b]
    \centering
    \begin{tikzpicture}[scale=0.65]
        \begin{axis}[x=4mm,
            ybar,
            ymin=0,
            ymax=40,
            ylabel=Frequency,
            xlabel=Dataset,
            xtick=data,
            x tick label style={rotate=45,anchor=east,font=\small},
            xtick align=inside,
            bar width=7.5pt,
            enlarge x limits=0.05,
            legend style={at={(0.5,-0.15)},
                anchor=north,legend columns=-1},
            symbolic x coords={Amazon,MovieLens,Tiktok,Yelp,Kwai,Taobao,Pinterest,UT-Zappos50K,MIND,Last.fm,Allrecipes,WeChat,Netflix Prize,FashionVC,POG,IQON3000,bodyFashion,Recipe1M+,Foodrec,MM-Rec,YouTube,Sharee/Lemon8,Dianping,Netflix Crawled,Polyvore,MSD-A,MM-INS
},
        ]
            \addplot[style = {fill=pallidyellow}] table [x=Dataset,y=Frequency,col sep=comma] {figures/datasets_frequency.csv};
        \end{axis}
    \end{tikzpicture}
    \caption{Frequency of multimodal datasets usage in multimodal recommender system papers published between 2017 and 2024.} 
    \label{fig:histogram_datasets}
\end{figure}



==> figures/modality_frequency.tex <==
\begin{figure}[t]
\subfloat[Visual Models]{
\begin{tikzpicture}[scale=0.8]
        \begin{axis}[
            width=5cm, 
            height=6cm,
            ylabel={Frequency},
            ybar,
            ymin=0,
            ymax=13,
            xtick=data,
            x tick label style={rotate=60,anchor=east,font=\small,text width=3cm, align=right},
            xtick align=inside,
            bar width=5pt,
            enlarge x limits=0.10,
            legend style={at={(0.5,-0.15)},
                anchor=north,legend columns=-1},
            symbolic x coords={
            ResNet,AlexNet,VGG,Custom,C3D,CLIP,GoogLeNet,Inception ResNet V2,Inception V3,Inception V4,Mask RCNN,ViLBERT}]
            \addplot[style = {fill=Mahogany}] table [x=Models,y=Frequency,col sep=comma] {figures/visual_frequency.csv};
        \end{axis}
    \end{tikzpicture}
}\subfloat[Textual Models]{
    \begin{tikzpicture}[scale=0.8]
        \begin{axis}[
            width=6cm, 
            height=6cm,
            ybar,
            ymin=0,
            ymax=13,
            xtick=data,
            x tick label style={rotate=60,anchor=east,font=\small,text width=3cm, align=right},
            xtick align=inside,
            bar width=5pt,
            enlarge x limits=0.10,
            legend style={at={(0.5,-0.15)},
                anchor=north,legend columns=-1},
            symbolic x coords={Custom,Sentence-BERT,TextCNN,CNN,GloVe,Sentence2Vec,Word2Vec,Bag-of-word scheme,BERT,BiLSTM,KimCNN,LDA,PV-DM,SIF,ViLBERT}]
            \addplot[style = {fill=RoyalBlue}] table [x=Models,y=Frequency,col sep=comma] {figures/textual_frequency.csv};
        \end{axis}
    \end{tikzpicture}
}\subfloat[Audio Models]{
\begin{tikzpicture}[scale=0.8]
        \begin{axis}[
            width=3cm, 
            height=6cm,
            ybar,
            ymin=0,
            ymax=13,
            xtick=data,
            x tick label style={rotate=60,anchor=east,font=\small,text width=3cm, align=right},
            xtick align=inside,
            bar width=5pt,
            enlarge x limits=1,
            legend style={at={(0.5,-0.15)},
                anchor=north,legend columns=-1},
            symbolic x coords={VGGish,Custom}]
            \addplot[style = {fill=OliveGreen}] table [x=Models,y=Frequency,col sep=comma] {figures/audio_frequency.csv};
        \end{axis}
    \end{tikzpicture}
}
\caption{Frequency of multimodal extractors usage in multimodal recommender system papers published between 2017 and 2024.}
\label{fig:extractor_histogram}
\end{figure}


==> figures/paper_domain.tex <==
\begin{figure}
    \centering
    \begin{tikzpicture}
    \begin{axis}[
        ybar,
        symbolic x coords={
            Collaborative,
            Context,
            Cross-domain,
            Federated,
            Graph,
            Knowledge,
            LLM,
            Multimodal,
            Sequential,
            Session
        },
        xtick=data,
        xticklabel style={rotate=35, anchor=north east},
        ylabel={Number of Papers},
        xlabel={Research Domain},
        ymin=0,
        bar width=14pt,
        enlarge x limits=0.12,
        nodes near coords,
        nodes near coords align={vertical},
        nodes near coords style={font=\scriptsize, text=black},
        ymajorgrids=true,
    ]

    \addplot+[draw=none, fill=semBrightGreen] coordinates {
        (Collaborative,32)
        (Context,42)
        (Cross-domain,83)
        (Federated,37)
        (Graph,71)
        (Knowledge,35)
        (LLM,39)
        (Multimodal,45)
        (Sequential,22)
        (Session,40)
    };

    \end{axis}
    \end{tikzpicture}
    \caption{Distribution of surveyed papers across research domains.}
    \label{fig:paper_domain_distribution}
\end{figure}

==> figures/paper_year.tex <==
\begin{figure}
    \centering
    \begin{tikzpicture}
    \begin{axis}[
        ybar,
        symbolic x coords={2001-06,2007-13,2014-19,2020-25},
        xtick=data,
        xticklabel style={anchor=north},
        ylabel=Frequency,
        xlabel=Publication Period,
        ymin=0,
        ymax=250,
        bar width=17pt,
        enlarge x limits=0.12,
        nodes near coords,
        nodes near coords style={font=\scriptsize, text=black},
        nodes near coords align={vertical},
    ]

    \addplot+[draw=none, fill=semBrightGreen] coordinates {
        (2001-06,2)
        (2007-13,34)
        (2014-19,190)
        (2020-25,219)
    };

    \end{axis}
    \end{tikzpicture}
    \caption{Temporal distribution of the collected papers grouped by publication period.}
    \label{fig:paper_year}
\end{figure}

==> figures/papers_rank.tex <==
% \begin{figure}[!t]
% \centering
% \begin{tikzpicture}
% \begin{axis}[
%     ybar, 
%     xlabel=Ranking,
%     ylabel=Frequency, 
%     xtick={1,2,3,4,5,6,7,8,9},
%     xticklabels={A*,A,B,C,Q1,Q2,Q3,WS,NR},
%     xtick style={draw=none},
%     xticklabel style={anchor=north},
%     enlarge x limits=0.15,
%     ymin=0,
%     nodes near coords,
%     nodes near coords align={vertical},
%     ylabel style={align=center}
% ]
% \addplot
% coordinates {
%     (1, 185)
%     (2, 51)
%     (3, 23)
%     (4, 2)
%     (5, 65)
%     (6, 10)
%     (7, 3)
%     (8, 14)
%     (9, 56)
% };

% \end{axis}
% \end{tikzpicture}
% \caption{}
% \label{fig:frequency}
% \end{figure}
\begin{figure}
    \centering
        \begin{tikzpicture}
        \begin{axis}[
            symbolic x coords={A*,A,B,C,Q1,Q2,Q3,WS,NR},
            xtick={A*,A,B,C,Q1,Q2,Q3,WS,NR},
            xticklabel style={anchor=north},
            ylabel=Frequency,
            ymin=0,
            ymax=210,
            bar width=17pt,
            enlarge x limits=0.12,
            nodes near coords,
            nodes near coords style={font=\scriptsize, text=black},
            nodes near coords align={vertical},
        ]
        \addplot[ybar, bar shift=0pt, draw=none, fill=semBrightGreen] coordinates {(A*,185)};
        \addplot[ybar, bar shift=0pt, draw=none, fill=semGreen]       coordinates {(A,51)};
        \addplot[ybar, bar shift=0pt, draw=none, fill=semYellow]      coordinates {(B,23)};
        \addplot[ybar, bar shift=0pt, draw=none, fill=semOrange]      coordinates {(C,2)};
        \addplot[ybar, bar shift=0pt, draw=none, fill=semBrightGreen] coordinates {(Q1,65)};
        \addplot[ybar, bar shift=0pt, draw=none, fill=semYellow]      coordinates {(Q2,10)};
        \addplot[ybar, bar shift=0pt, draw=none, fill=semOrange]      coordinates {(Q3,3)};
        \addplot[ybar, bar shift=0pt, draw=none, fill=cyan]           coordinates {(WS,14)};
        \addplot[ybar, bar shift=0pt, draw=none, fill=semGray]        coordinates {(NR,56)};

        \end{axis}
        \end{tikzpicture}
    \caption{Caption}
    \label{fig:papers_rank}
\end{figure}

==> sections/case_study.tex <==
\chapter{Case Study: the Gowalla Dataset}

Qui per concludere mettiamo l'esempio del tutorial

\section{Reproducible Multimodal Feature Extraction in Recommendation Experiments}
\label{subsec:feat_reproducibility}
\angela{alberto aveva detto che questa sezione è da spostare?}

Reproducibility at this stage requires, for each modality, five elements to be fully documented: the raw input source (e.g., which image URLs, video files, or textual fields are used); the preprocessing pipeline (tokenisation and normalisation for text; frame sampling, resizing, and normalisation for images and video; track extraction and time--frequency transformation for audio); the encoder architecture and exact checkpoint; the strategy used to obtain a single item-level embedding from multiple modality-specific fragments; and either public extraction code or pre-computed representations. Without all five, the feature space on which a model is trained cannot be faithfully reconstructed by external researchers.

We find that many of the reported papers satisfy at most the first of these requirements, naming the encoder family but omitting the remaining steps.

For \emph{text}, most works report only a high-level label (GloVe, BERT, Sentence-BERT, or Sentence2Vec) without specifying the pretrained checkpoint, tokeniser, sequence length, or pooling rule. In \citeauthor{DBLP:conf/cikm/KimLSK22}'s \textsc{mario} model, for instance, item text is embedded with Sentence-BERT, but the specific Sentence-BERT checkpoint, the exact textual fields used, and the aggregation of multiple texts per item are not detailed~\citep{DBLP:conf/cikm/KimLSK22}. Similarly, \citeauthor{DBLP:conf/www/Han0NL22} build their modality-disentangled pretraining objectives on top of VGG-19 and GloVe embeddings without fixing the GloVe variant, tokenisation, or sentence-level aggregation strategy~\citeauthor{DBLP:conf/www/Han0NL22}, and \citeauthor{DBLP:journals/tmm/LiuCCLNK23} rely on a review encoder that is described only at a conceptual level, with no concrete language-model checkpoint or preprocessing detail~\citep{DBLP:journals/tmm/LiuCCLNK23}. A positive outlier is \textsc{mm-rec}~\citep{DBLP:conf/sigir/WuWQZHX22}, which encodes news text and images jointly through VilBERT and is accompanied by publicly available code that implements the ROI extraction and encoding.

The picture for \emph{visual and video} features is analogous. Works routinely cite a backbone (ResNet-50, VGG-16/19, Inception-v3/v4, or ViT) without disclosing image resolution, normalisation, frame-sampling rate, or the source of the checkpoint. \citeauthor{DBLP:journals/isci/NiHHL22}, for example, feed CNN-based image features (e.g., from ResNet-50) into their two-stage embedding model on MovieLens-20M and Book-Crossing but do not specify how many images per item are used, at what resolution they are processed, or which pretrained weights are loaded~\citep{DBLP:journals/isci/NiHHL22}. An exception are micro-video datasets such as TikTok and Kwai: since the competition organisers release pre-computed multimodal features that subsequent works such as \textsc{mmgcn} and \textsc{dualgnn} consume directly (family (d) of \Cref{subsec:feat_taxonomy}), feature-extraction reproducibility is in fact guaranteed for these datasets~\citep{DBLP:conf/mm/WeiWN0HC19, DBLP:journals/tmm/WangWYWSN23}---though, as noted above, at the cost of encoder visibility. \textsc{mm-rec} sets a higher bar by describing Mask R-CNN region-of-interest detection and its integration with VilBERT, and by releasing the corresponding implementation~\citep{DBLP:conf/sigir/WuWQZHX22}.

For \emph{audio}, the gap is widest. Only a few surveyed works include audio input, almost always via 128-dimensional VGGish embeddings from video soundtracks, and in most cases the description stops at naming the backbone. \citeauthor{DBLP:conf/mm/LiuYLWTZSM21} explicitly mention extracting audio from MovieLens trailers with \texttt{ffmpeg} and then applying VGGish, but do not report the \texttt{ffmpeg} settings, the VGGish checkpoint, or the temporal segmentation and pooling scheme~\citep{DBLP:conf/mm/LiuYLWTZSM21}. In the micro-video setting, \textsc{mmgcn}, \textsc{dualgnn}, and \textsc{mgat} all treat VGGish features as a pre-computed acoustic modality on TikTok, consuming the fixed vectors released with the dataset, while on MovieLens they follow an MMGCN-style pipeline from trailers to VGGish embeddings without fully specifying its parameters~\citep{DBLP:conf/mm/WeiWN0HC19, DBLP:journals/tmm/WangWYWSN23}.

Taken together, these examples show that, for all three modalities, feature pipelines are still mostly treated as background implementation choices.


==> sections/current_trends.tex <==
\chapter{Overview of Data Handling and Processing in Recommender Systems}
\input{tables/literature}

Managing and processing recommendation datasets is a fundamental aspect of recommender system research, yet strategies can vary significantly across studies. 
To capture the current landscape, we examined recent papers published at leading conferences in information retrieval and recommender systems, with a focus on the data-handling strategies adopted in their experimental pipelines. 
This analysis highlights prevailing practices in data management and preprocessing for recommendation research and sheds light on commonalities, divergences, and open challenges in the field.

\section{Current Trends in Recommender Research}

Techniques and procedures for data handling in recommender systems are diverse and often depend on the specific dataset, domain, or research objective. To identify the most commonly adopted approaches, we analyzed 55 papers published between 2020 and 2024, extracted from five surveys covering different areas of recommendation research: \textbf{graph neural networks}~\cite{DBLP:journals/csur/WuSZXC23}, \textbf{contrastive learning}~\cite{DBLP:journals/tois/JingZZW24}, \textbf{temporal modeling}~\cite{DBLP:journals/umuai/BoginaKJBKT23}, \textbf{reinforcement learning}~\cite{DBLP:journals/csur/AfsarCF23}, and \textbf{generative approaches}~\cite{DBLP:journals/corr/abs-2404-00579}. 
The selection of these papers ensures relevance to the community, coverage of diverse domains, and representation of state-of-the-art research. 
\Cref{tab:papers_datasets_complete} summarises the results of our analysis.

Acknowledging the heterogeneity of current practices, this survey provides a comprehensive overview of dataset usage, filtering strategies, and data-splitting methods adopted in recent studies, and discusses their broader implications for the reproducibility of recommender systems research. 
In the following sections, we present the results of this systematic investigation, highlighting differences in dataset selection, binarisation, and filtering techniques, as well as evaluation protocols.


\subsection{Datasets}

\input{tables/how_datasets_are_referred}
The surveyed papers reveal a remarkable breadth in dataset usage, with \textbf{79 distinct datasets} identified. 
Within these, the ones appearing in at least three different datasets are explicitly reported in~\Cref{tab:papers_datasets_complete}.
This extensive utilisation of diverse datasets underscores the inherent adaptability and domain-agnostic nature of recommender systems, showcasing their capacity to address a wide array of real-world applications. 
Indeed, this heterogeneity reflects the field's maturity and its responsiveness to varied application contexts. 

However, our review raises a significant issue in how recommendation datasets are referenced, as evidenced by the further analysis reported in~\Cref{tab:dataset_references}.

While papers using open datasets should reference the \textbf{original data source}, only 35.2\% of the 179 dataset usages analysed provide such an explicit reference.
Among the remaining cases, 32.4\% fail to cite the source entirely, instead offering a \textbf{copy of a new version of the dataset}---often already processed---without clarifying its origin. Although this practice may support reproducibility, it does not ensure a clear reproduction of the filtering methods applied, compromising the validation of these approaches.
Additionally, 16.8\% cite only the \textbf{dataset's original paper} or \textbf{other scholarly papers}, which does not guarantee clarity about the dataset used, especially when multiple online versions exist.
Finally, 15.6\% of the datasets are irretrievable, either due to the \textbf{absence of any reference} or because the provided \textbf{links are broken}, e.g, they are no longer functional or have been blocked.

This analysis highlights the importance of tracking and versioning recommendation datasets.~\cite{DBLP:conf/kars/PaparellaMFPAN23} By maintaining a direct reference to the original or trusted sources and by providing tools to reproduce filtering and splitting approaches, complete reproducibility can be ensured. For this reason, \datarec includes classes and methods for direct and traceable management of the most widely used datasets in the analysed papers, specifically, those appearing in at least three different articles, as reported in~\Cref{tab:papers_datasets_complete}.

\subsection{Binarization and Filtering}
Preprocessing strategies are critical in every experimental setting, as meaningful evaluations require aligning datasets with the experimental design. Consequently, ensuring the reproducibility of these strategies is essential for valid comparisons across different experiments. Our analysis identified the most commonly adopted approaches, retaining only those that appear in at least three datasets, which are reported in~\Cref{tab:papers_datasets_complete}.

One fundamental preprocessing strategy is \textbf{binarisation}, which converts explicit feedback into implicit feedback. 
This transformation facilitates the training and evaluation of models that estimate the likelihood of interactions rather than predicting exact rating values. This task has become increasingly prevalent in contemporary recommender systems~\cite{DBLP:conf/uai/RendleFGS09,DBLP:conf/icdm/HuKV08,DBLP:conf/recsys/TakacsPT11, DBLP:conf/irongraphs/BufiMFMNS24, DBLP:journals/tors/FerraraAMNS23}. 

Another widely employed strategy is the \textbf{$k$-core} filtering method, used to remove users (\textbf{$k$-Core User}), items (\textbf{$k$-Core Item}), or iteratively both (\textbf{$k$-Core Iterative}). Interactions below the threshold are often considered too sparse or noisy to provide reliable preference signals and are therefore excluded to prevent them from negatively affecting model performance. 

Additional filtering strategies appear in session-based recommendation experiments, where data may be filtered according to \textbf{session length}, e.g., by discarding sessions that are too short or excessively long. These methods, while less general, have been increasingly adopted in recent work on sequential and session-based recommendation.


\subsection{Splitting}
Data splitting strategies partition datasets into training, validation, and test sets, and are a critical component of experimental design. 
Our survey confirms prior findings~\cite{DBLP:conf/recsys/MengMMO20, DBLP:conf/sigir/Sun23} that there is no universally accepted splitting method. 
Instead, studies employ diverse strategies, often without explicit justification, which contributes to inconsistent rankings of recommender systems even when the same datasets and metrics are used~\cite{DBLP:conf/recsys/DacremaCJ19, DBLP:journals/csur/ZhangYST19}.

The most commonly observed strategies, summarized in~\Cref{tab:papers_datasets_complete}, include:
\begin{itemize}
    \item \textbf{Random Holdout Splitting}: Randomly partitions the dataset into training, validation, and test sets based on predefined percentages. This remains the most common approach.
    \item \textbf{Temporal Leave-1-Out}: Extracts the last interaction per user for the test set and one preceding interaction for validation. This is the second most common strategy.
    \item \textbf{Random Leave-1-Out}: Similar to the temporal variant, but the interaction selected for testing is chosen randomly from the user history.
    \item \textbf{Pre-computed Splits}: Some studies rely on dataset versions where train, validation, and test splits are already provided.
    \item \textbf{Temporal Fixed}: Partitions data based on timestamps, either globally (e.g., all interactions after a fixed time point) or per user (e.g., a percentage of the most recent interactions).
    % \item \textbf{Cross Validation}: Less frequent; divides the dataset into multiple folds, iteratively rotating which fold is used for testing.
\end{itemize}

This variety of strategies highlights the lack of consensus in the community and underscores the need for more transparent reporting and systematic evaluation of splitting methods, given their strong influence on the reproducibility and comparability of experimental results.

==> tables/datasets.tex <==
\hypersetup{
    colorlinks=true, 
    urlcolor=Purple
}

\begin{table}[!t]
\centering
\caption{Overview of multimodal recommendation datasets, detailing crucial features such as publication year, domain classification, incorporated modalities (visual, textual, audio),  original and pre-processed data availability, and public accessibility.}

\begin{adjustbox}{width=\textwidth, center}
\rowcolors{2}{gray!17.5}{white}
\begin{tabular}{lcccccccc}
\toprule
\textbf{Datasets} & \textbf{Year} &
\textbf{Domain} &
\multicolumn{3}{c}{\textbf{Modalities}} & \multicolumn{2}{c}{\textbf{Data}} & \textbf{Publicly available} \\
\cmidrule(lr){4-6} \cmidrule(lr){7-8}
 \multicolumn{ 1}{c}{}  & \multicolumn{ 1}{c}{}  & & \multirow{1}{*}{\textcolor{Mahogany}{Visual}} & \multirow{1}{*}{\textcolor{RoyalBlue}{Textual}} & \multirow{1}{*}{\textcolor{OliveGreen}{Audio}} & Original & Pre-processed & \\
\midrule
        %Rec-TMALL~\cite{DBLP:journals/corr/ZhangPSW14, DBLP:conf/kdd/ZhongJYYZL15} & {2014}  & Fashion & \cmark & \cmark &  &  \cmark & & \href{https://tianchi.aliyun.com/dataset/43}{\textbf{[link]}} \\
        UT Zappos50K~\cite{DBLP:conf/cvpr/YuG14, DBLP:conf/iccv/YuG17} & 2014 & Fashion & \cmark & \cmark & & \cmark & \cmark & \href{https://vision.cs.utexas.edu/projects/finegrained/utzap50k/}{\textbf{[link]}} \\
        FashionVC~\cite{DBLP:conf/mm/SongFLLNM17} &  {2017}  & Fashion & \cmark & \cmark &   & \cmark & & \href{https://drive.google.com/file/d/1d72E3p4w280-vdCKfXtXZLMULpIScRRR/view?usp=sharing}{\textbf{[link]}} \\
        Polyvore~\cite{han2017learning} & 2017 & Fashion & \cmark & \cmark &  & \cmark & & \href{https://github.com/xthan/polyvore-dataset}{\textbf{[link]}} \\
        Taobao~\cite{Taobao} & 2018 & Fashion & \cmark & \cmark &  & \cmark & & \href{https://tianchi.aliyun.com/dataset/52}{\textbf{[link]}} \\
        POG~\cite{DBLP:conf/kdd/ChenHXGGSLPZZ19} & {2019}  & Fashion & \cmark & \cmark &  & \cmark & & \href{https://github.com/wenyuer/POG}{\textbf{[link]}} \\
        IQON3000~\cite{DBLP:conf/mm/SongHLCXN19} & 2019 & Fashion & \cmark & \cmark &  & \cmark & \cmark & \href{https://anonymity2019.wixsite.com/gp-bpr}{\textbf{[link]}} \\
        bodyFashion~\cite{DBLP:conf/mm/DongSFJXN19} & 2019 & Fashion & \cmark & \cmark &  & \cmark &  & \href{https://dxresearch.wixsite.com/pcw-dc}{\textbf{[link]}} \\ \midrule

        Last.fm\footnote{\url{http://www.lastfm.com}}~\cite{Cantador:RecSys2011} & 2011 & Music & \cmark & \cmark & \cmark  & \cmark & & \href{https://www.heywhale.com/mw/dataset/5cfe0526e727f8002c36b9d9/content}{\textbf{[link]}} \\ 
        MSD-A~\cite{DBLP:conf/recsys/OramasNSS17} & 2017 & Music &  & \cmark & \cmark & \cmark & \cmark &  \href{https://www.upf.edu/web/mtg/msd-a}{\textbf{[link]}} \\
        WeChat~\cite{DBLP:conf/ijcnn/Shen0LWC20}& 2020 & Music & \cmark & \cmark & \cmark  & & & \xmark \\ \midrule

        Amazon Review~\cite{DBLP:conf/emnlp/NiLM19} & 2013-2023 & E-commerce & \cmark & \cmark &   & \cmark & & \href{https://cseweb.ucsd.edu/~jmcauley/datasets/amazon\_v2/}{\textbf{[link]}} \\ \midrule
        
        Recipe1M+~\cite{marin2019learning, salvador2017learning} & 2017 & Recipe & \cmark & \cmark &   & \cmark & \cmark & \href{http://im2recipe.csail.mit.edu/}{\textbf{[link]}} \\
        FoodRec~\cite{DBLP:conf/mm/JiangW0NDX19} & 2019 & Recipe & \cmark & \cmark &   & & \cmark & \href{https://acmmultimedia.wixsite.com/foodrec}{\textbf{[link]}} \\
        Allrecipes~\cite{DBLP:journals/tmm/GaoFHHGFMC20} & 2020 & Recipe & \cmark & \cmark &   & \cmark & & \href{https://www.kaggle.com/datasets/elisaxxygao/foodrecsysv1}{\textbf{[link]}} \\ \midrule

        MIND~\cite{DBLP:conf/acl/WuQCWQLLXGWZ20} & 2020 & News & \cmark & \cmark &   & & \cmark & \href{https://msnews.github.io/}{\textbf{[link]}} \\
        MM-Rec~\cite{DBLP:conf/sigir/WuWQZHX22} & 2022 & News & \cmark & \cmark &   & \cmark &  & \href{https://github.com/zcfinal/MM-Rec}{\textbf{[link]}} \\ 
        %EB-NeRD & 2024 & News & \cmark & \cmark &   & & \cmark & \href{https://recsys.eb.dk/}{\textbf{[link]}} \\ 
        \midrule

        % Book-Crossings & 2004 & Book & \cmark & \cmark &   & & \cmark & ??\href{https://www.kaggle.com/datasets/ignacioavas/alignmacrid-vae}{\textbf{[link]}} \\ \midrule

        Pinterest~\cite{DBLP:conf/iccv/GengZBC15}& 2015 & Social Media & \cmark & \cmark & & \cmark &  & \href{https://github.com/edervishaj/pinterest-recsys-dataset?tab=readme-ov-file}{\textbf{[link]}} \\
        %AudioSet~\cite{DBLP:conf/icassp/GemmekeEFJLMPR17}& 2017 & Social Media &  &  & \cmark & & \cmark & \href{https://research.google.com/audioset/download.html}{\textbf{[link]}} \\
        Kwai~\cite{DBLP:journals/corr/abs-2009-06573} & {2020} & Social Media & \cmark & \cmark &   & & \cmark & \href{https://zenodo.org/record/4023390\#.Y9YZ6XZBw7c}{\textbf{[link]}} \\
        MM-INS~\cite{DBLP:journals/tcss/YangWLLGDW20} & 2020 & Social Media & \cmark & \cmark &   & \cmark & & \href{https://github.com/w5688414/AMNN}{\textbf{[link]}} \\
        Youtube~\cite{DBLP:journals/tmm/SangXQMLW21} & 2021 & Social Media & \cmark & \cmark & & & & \xmark \\
        Sharee/Lemon8~\cite{DBLP:conf/mir/LiuMSO022} & 2021  & Social Media & \cmark & \cmark &  & & & \xmark \\ 
        TikTok & 2023  & Social Media & \cmark & \cmark & \cmark  &  & \cmark & \href{https://drive.google.com/drive/folders/1AB1RsnU-ETmubJgWLpJrXd8TjaK_eTp0}{\textbf{[link]}} \\ \midrule

        Dianping~\cite{LiLMR20, LiLQMTC19, LiWTM15, LiWM14} & 2020 & Restaurant & \cmark & \cmark &   & & & \href{https://lihui.info/data/dianping/}{\textbf{[link]}} \\
        Yelp & 2013-2023 & Restaurant & \cmark & \cmark &  & \cmark & & \href{https://www.yelp.com/dataset}{\textbf{[link]}} \\ \midrule

        Movielens & 1997-2021 & Movie & & \cmark & & \cmark & & \href{https://grouplens.org/datasets/movielens/}{\textbf{[link]}} \\
        Netflix Prize data \cite{Bennett2007TheNP} & 2007  & Movie &  & \cmark &   & & & \href{https://www.kaggle.com/datasets/netflix-inc/netflix-prize-data}{\textbf{[link]}} \\
        Netflix Crawled \cite{wei2023multi} &  2023 & Movie & \cmark & \cmark &  & \cmark & \cmark & \href{https://drive.google.com/drive/folders/1BGKm3nO4xzhyi_mpKJWcfxgi3sQ2j_Ec}{\textbf{[link]}} \\
\bottomrule
\end{tabular}
\end{adjustbox}
\label{tab:datasets}
\end{table}


==> tables/how_datasets_are_referred.tex <==
\begin{table}[h]
\centering
\caption{Dataset referencing in surveyed papers. The table reports the different ways datasets are cited, including references to the original data source, copies of the dataset, citations of the dataset’s original paper or other scholarly papers, missing references, and broken links.}
\begin{tabular}{l c}
\toprule
\textbf{Reference Type}                     & \textbf{\# Usages (Percentage)} \\ \midrule
Original data source     & 63 (35.2\%)                      \\
Copy a new version of the dataset         & 58 (32.4\%)                      \\
Dataset's original paper           & 27 (15.1\%)                      \\
Other scholarly papers             & 3 (1.7\%)                        \\
No reference                          & 19 (10.6\%)                      \\
Broken link             & 9 (5.0\%)                        \\ \midrule
\textbf{Total}                        & \textbf{179 (100\%)}             \\ \bottomrule
\end{tabular}
\label{tab:dataset_references}
\end{table}

==> tables/literature.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
\begin{table*}[]
\centering
\caption{Datasets, pre-processing and splitting strategies adopted in 55 research papers published between 2020 and 2024. Only datasets and strategies appearing in at least 3 research papers are shown.}
\label{tab:papers_datasets_complete}
  \rowcolors{2}{white}{gray!25}
  %\newcolumntype{a}{>{\columncolor{red}}c}
  \setlength{\tabcolsep}{3.3pt}
  \footnotesize
\begin{tabular}{*{3}{l}@{\hskip 1.5em}*{16}{c}@{\hskip 1.5em}*{7}{c}@{\hskip 1.5em}*{7}{c}}
    \toprule
                                    &               &                                                     & \multicolumn{16}{c}{\textbf{Datasets}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                          & \multicolumn{7}{c}{\textbf{Pre-processing}}                                                                                                                                                                                                                                                                                                  & \multicolumn{7}{c}{\textbf{Splitting}}                                                                                                                                                                                                                                                                                                                                           \\
        \cmidrule(r){4-19} \cmidrule(lr){20-26} \cmidrule(l){27-33}                                    
                \textbf{Paper}   & \textbf{Venue} & \textbf{Year}                                      & \rotatebox{90}{\textbf{Yelp}} & \rotatebox{90}{\textbf{Amazon Books}} & \rotatebox{90}{\textbf{MovieLens 1M}} & \rotatebox{90}{\textbf{Amazon Beauty}} & \rotatebox{90}{\textbf{Last.fm}} & \rotatebox{90}{\textbf{Gowalla}} & \rotatebox{90}{\textbf{Amazon Toys and Games}} & \rotatebox{90}{\textbf{Tmall}} & \rotatebox{90}{\textbf{Amazon Games}} & \rotatebox{90}{\textbf{Yelp2018}} & \rotatebox{90}{\textbf{Alibaba-iFashion}} & \rotatebox{90}{\textbf{Amazon Clothing}} & \rotatebox{90}{\textbf{Amazon Sports and Outdoors}} & \rotatebox{90}{\textbf{Epinions}} & \rotatebox{90}{\textbf{MovieLens 20M}} & \rotatebox{90}{\textbf{\textit{Others}}} & \rotatebox{90}{\textbf{\textit{None}}} & \rotatebox{90}{\textbf{Binarization}} & \rotatebox{90}{\textbf{$k$-Core Iterative}} & \rotatebox{90}{\textbf{$k$-Core User}} & \rotatebox{90}{\textbf{$k$-Core Item}} & \rotatebox{90}{\textbf{Session length}} & \rotatebox{90}{\textbf{\textit{Others}}} & \rotatebox{90}{\textbf{Random Hold-Out}} & \rotatebox{90}{\textbf{Temporal Leave-1-out Hold-Out}} & \rotatebox{90}{\textbf{Fixed}} & \rotatebox{90}{\textbf{Random Leave-1-out Hold-Out}} & \rotatebox{90}{\textbf{Temporal Fixed Handcrafted}} & \rotatebox{90}{\textbf{\textit{Others}}} & \rotatebox{90}{\textbf{\textit{NA}}} \\
                   \midrule 
\cite{DBLP:journals/tois/HaoYZLC23}       & TOIS      & 2023 &        &        & \cmark &        &        & \cmark &        &        &        &        &        &        &        &        &        & \cmark & \cmark &        &        &        &        &        &        & \cmark &        &        &        &        &        &        \\
\cite{DBLP:conf/sigir/ShuaiZWSHWL22}      & SIGIR     & 2022 & \cmark &        &        &        &        &        & \cmark &        &        &        &        & \cmark &        &        &        & \cmark &        &        &        & \cmark &        &        &        & \cmark &        &        &        &        &        &        \\
\cite{DBLP:conf/kdd/Jiang0H23}            & KDD       & 2023 & \cmark &        &        &        & \cmark &        &        &        &        &        &        &        &        &        &        & \cmark & \cmark &        & \cmark &        &        &        &        & \cmark &        &        &        &        &        &        \\
\cite{DBLP:conf/sigir/YuY00CN22}          & SIGIR     & 2022 &        & \cmark &        &        &        &        &        &        &        & \cmark &        &        &        &        &        & \cmark & \cmark & \cmark &        &        &        &        &        & \cmark &        &        &        &        &        &        \\
\cite{DBLP:conf/www/XiaHHLYK23}           & WWW       & 2023 & \cmark & \cmark &        &        &        & \cmark &        &        &        &        &        &        &        &        &        &        & \cmark &        &        &        &        &        &        & \cmark &        &        &        &        &        &        \\
\cite{DBLP:conf/recsys/Hansen0MMBTL20}    & RecSys    & 2020 &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        & \cmark & \cmark &        &        &        &        &        &        &        &        &        &        & \cmark &        &        \\
\cite{DBLP:conf/cikm/0158ZLYY22}          & CIKM      & 2022 &        &        &        & \cmark &        &        & \cmark &        &        &        &        &        &        &        &        & \cmark &        & \cmark & \cmark &        &        &        &        &        & \cmark &        &        &        &        &        \\
\cite{DBLP:journals/tcyb/FuAIZHQ22}       & Cyb IEEE  & 2021 &        &        & \cmark &        &        &        &        &        &        &        &        &        &        &        & \cmark & \cmark &        & \cmark &        & \cmark &        &        &        &        &        &        &        &        & \cmark &        \\
\cite{DBLP:conf/mm/Wu0CLHS023}            & MM        & 2023 & \cmark &        & \cmark & \cmark &        &        &        &        &        &        &        &        &        &        &        & \cmark &        & \cmark &        & \cmark &        &        &        &        & \cmark &        &        &        &        &        \\
\cite{DBLP:conf/sigir/WangXFL0C23}        & SIGIR     & 2023 & \cmark & \cmark & \cmark &        &        &        &        &        &        &        &        &        &        &        &        &        &        & \cmark &        &        &        &        &        & \cmark &        &        &        &        &        &        \\
\cite{DBLP:conf/sigir/RenXZY023}          & SIGIR     & 2023 &        & \cmark &        &        &        & \cmark &        & \cmark &        &        &        &        &        &        &        &        & \cmark &        &        &        &        &        &        &        &        & \cmark &        &        &        &        \\
\cite{DBLP:conf/cikm/ZhangGYGLY21}        & CIKM      & 2021 &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        & \cmark & \cmark & \cmark &        &        &        &        & \cmark & \cmark &        &        &        &        &        &        \\
\cite{DBLP:conf/kdd/GuoSTGZLTH21}         & SIGKDD    & 2021 &        &        &        &        &        &        &        & \cmark &        &        &        &        &        &        &        & \cmark & \cmark &        &        &        &        &        &        &        &        &        & \cmark &        &        &        \\
\cite{DBLP:journals/tkde/ZhangWYLW23}     & TKDE      & 2022 &        &        &        & \cmark &        &        &        &        & \cmark &        &        &        &        &        &        & \cmark &        &        & \cmark &        &        &        &        &        & \cmark &        &        &        &        &        \\
\cite{DBLP:conf/sigir/DuYZZ00LS23}        & SIGIR     & 2023 &        &        & \cmark & \cmark &        &        & \cmark &        &        &        &        &        &        &        &        &        &        & \cmark &        &        &        &        &        &        & \cmark &        &        &        &        &        \\
\cite{DBLP:conf/icde/Xie0YYGO021}         & ICDE      & 2021 &        &        & \cmark & \cmark &        &        &        &        & \cmark &        &        &        &        &        & \cmark &        &        & \cmark &        &        &        &        & \cmark &        & \cmark &        &        &        &        &        \\
\cite{DBLP:journals/tkde/HaoZZLSXLZ23}    & TKDE      & 2023 &        &        &        &        &        &        & \cmark & \cmark &        &        &        &        &        &        &        &        &        &        &        & \cmark & \cmark &        &        &        & \cmark &        &        &        &        &        \\
\cite{DBLP:conf/recsys/0008P020}          & RecSys    & 2020 &        &        &        & \cmark &        &        &        & \cmark & \cmark &        &        &        &        &        &        & \cmark &        & \cmark & \cmark &        &        &        &        &        & \cmark &        &        &        &        &        \\
\cite{DBLP:conf/pkdd/JingZZYT22}          & PKDD      & 2022 &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        & \cmark & \cmark &        &        &        &        &        &        & \cmark &        &        &        &        &        &        \\
\cite{DBLP:journals/fcsc/WuHWWCLX22}      & FCS       & 2022 &        & \cmark &        &        &        &        &        &        &        &        &        &        &        &        &        & \cmark &        &        &        & \cmark &        &        &        &        & \cmark &        &        &        &        &        \\
\cite{DBLP:journals/tois/ZhangSYXOZ20}    & TOIS      & 2020 &        &        &        & \cmark & \cmark &        &        &        & \cmark &        &        &        &        &        & \cmark & \cmark &        & \cmark & \cmark & \cmark & \cmark &        & \cmark &        & \cmark &        &        &        & \cmark &        \\
\cite{DBLP:conf/www/XiaHSX23}             & WWW       & 2023 & \cmark & \cmark &        &        &        & \cmark &        &        &        &        &        &        &        &        &        &        & \cmark &        &        &        &        &        &        & \cmark &        &        &        &        &        &        \\
\cite{DBLP:conf/wsdm/ChenHXWXL23}         & WSDM      & 2023 & \cmark &        &        &        &        &        &        &        &        &        &        &        &        & \cmark &        & \cmark & \cmark &        &        &        &        &        &        &        &        &        & \cmark &        &        &        \\
\cite{DBLP:conf/sigir/XiaHXZYH22}         & SIGIR     & 2022 & \cmark & \cmark &        &        &        &        &        &        &        &        &        &        &        &        &        & \cmark & \cmark &        & \cmark &        &        &        &        & \cmark &        &        &        &        &        &        \\
\cite{DBLP:journals/eswa/BoginaVKD22}     & ESwA      & 2022 &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        & \cmark &        &        &        &        &        & \cmark & \cmark & \cmark &        &        &        &        &        &        \\
\cite{DBLP:conf/recsys/MancinoFBMNS23}    & RecSys    & 2023 &        &        & \cmark &        &        &        &        &        &        &        &        &        &        &        &        & \cmark &        & \cmark & \cmark &        &        &        &        & \cmark &        &        &        &        &        &        \\
\cite{DBLP:conf/sigir/YangHXL22}          & SIGIR     & 2022 &        & \cmark &        &        &        &        &        &        &        & \cmark &        &        &        &        &        & \cmark & \cmark &        &        &        &        &        &        &        &        & \cmark &        &        &        &        \\
\cite{DBLP:conf/kdd/YangHXH23}            & KDD       & 2023 &        &        &        &        & \cmark &        &        &        &        &        & \cmark &        &        &        &        & \cmark &        &        & \cmark &        &        &        &        & \cmark &        &        &        &        &        &        \\
\cite{DBLP:conf/wsdm/WangX0SLG023}        & WSDM      & 2023 &        & \cmark &        &        & \cmark &        &        &        &        &        &        &        &        &        &        & \cmark &        &        & \cmark &        &        &        &        & \cmark &        &        &        &        &        &        \\
\cite{DBLP:conf/aaai/HuangXXDXLBXLY21}    & AAAI      & 2021 & \cmark &        &        &        &        &        &        &        &        &        &        &        &        & \cmark &        & \cmark & \cmark &        &        &        &        &        &        &        &        &        & \cmark &        &        &        \\
\cite{DBLP:conf/sigir/TianXLYZ22}         & SIGIR     & 2022 & \cmark & \cmark & \cmark &        &        &        &        &        &        &        &        &        &        &        &        &        &        & \cmark & \cmark &        &        &        &        & \cmark &        &        &        &        &        &        \\
\cite{DBLP:conf/iclr/Cai0XR23}            & ICLR      & 2023 & \cmark & \cmark &        &        &        & \cmark &        & \cmark &        &        &        &        &        &        &        & \cmark & \cmark &        &        &        &        &        &        &        &        & \cmark &        &        &        &        \\
\cite{DBLP:conf/sigir/0001DWLZ020}        & SIGIR     & 2020 &        & \cmark &        &        &        & \cmark &        &        &        & \cmark &        &        &        &        &        &        & \cmark &        &        &        &        &        &        &        &        & \cmark &        &        &        &        \\
\cite{DBLP:conf/cikm/WangL0HMHFC22}       & CIKM      & 2022 &        & \cmark &        &        &        & \cmark & \cmark &        &        &        &        & \cmark &        &        &        &        &        &        &        &        & \cmark &        &        & \cmark &        &        &        &        &        &        \\
\cite{DBLP:conf/sigir/Zou0MWQ0C22}        & SIGIR     & 2022 &        &        & \cmark &        & \cmark &        &        &        &        &        &        &        &        &        &        & \cmark &        & \cmark &        &        &        &        &        & \cmark &        &        &        &        &        &        \\
\cite{DBLP:conf/www/WeiHXZ23}             & WWW       & 2023 &        &        &        &        &        &        &        &        &        &        &        &        & \cmark &        &        & \cmark & \cmark &        &        &        &        &        &        &        &        & \cmark &        &        &        &        \\
\cite{DBLP:conf/dasfaa/WuXZACZZLH22}      & DASFAA    & 2022 &        &        &        &        &        &        &        & \cmark &        &        &        &        &        &        &        &        &        &        & \cmark &        &        &        &        &        & \cmark &        &        &        &        &        \\
\cite{DBLP:journals/tois/LiZC23}          & SIGIR     & 2023 & \cmark &        &        &        &        &        &        &        &        &        &        &        &        &        &        & \cmark & \cmark &        &        &        &        &        &        &        &        &        &        &        & \cmark &        \\
\cite{DBLP:conf/nips/RajputMSKVHHT0S23}   & NIPS      & 2024 &        &        &        & \cmark &        &        & \cmark &        &        &        &        &        & \cmark &        &        &        &        &        &        & \cmark &        &        &        &        & \cmark &        &        &        &        &        \\
\cite{DBLP:conf/aaai/ChenWHZW20}          & AAAI      & 2020 &        & \cmark &        &        &        & \cmark &        &        &        &        &        &        &        &        &        &        &        &        & \cmark &        &        &        &        & \cmark &        &        &        &        &        &        \\
\cite{DBLP:conf/sigir/HadaMS21}           & SIGIR     & 2021 &        &        &        &        &        &        &        &        &        &        &        & \cmark &        &        &        & \cmark &        &        & \cmark &        &        &        &        &        &        &        &        &        & \cmark &        \\
\cite{DBLP:conf/cikm/ZhouWZZWZWW20}       & CIKM      & 2020 & \cmark &        &        & \cmark & \cmark &        & \cmark &        &        &        &        &        & \cmark &        &        & \cmark & \cmark &        &        &        &        &        &        &        & \cmark &        &        &        &        &        \\
\cite{DBLP:conf/cikm/0013YYSC21}          & CIKM      & 2022 &        &        &        &        &        &        &        & \cmark &        &        &        &        &        &        &        & \cmark &        &        &        &        & \cmark & \cmark &        &        &        &        &        & \cmark &        &        \\
\cite{DBLP:conf/sigir/WuWF0CLX21}         & SIGIR     & 2021 &        &        &        &        &        &        &        &        &        &        & \cmark &        &        &        &        &        &        &        &        &        &        &        & \cmark & \cmark &        &        &        &        &        &        \\
\cite{DBLP:conf/ijcai/GuWSX22}            & IJCAI     & 2022 & \cmark &        &        &        &        &        &        &        &        &        &        &        &        &        &        & \cmark & \cmark &        &        &        &        &        &        &        &        &        & \cmark &        &        &        \\
\cite{DBLP:conf/www/YuYLWH021}            & WWW       & 2021 & \cmark &        &        &        & \cmark &        &        &        &        &        &        &        &        &        &        & \cmark & \cmark & \cmark &        &        &        &        &        &        &        &        &        &        & \cmark &        \\
\cite{DBLP:conf/sigir/ChangGZHNSJ021}     & SIGIR     & 2021 &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        & \cmark &        &        & \cmark & \cmark &        &        &        &        &        &        &        & \cmark &        &        \\
\cite{DBLP:journals/isci/LatifiMJ21}      & Inf. Sci. & 2021 &        &        &        &        & \cmark &        &        &        &        &        &        &        &        &        &        & \cmark &        &        &        & \cmark &        & \cmark & \cmark &        &        &        &        &        & \cmark &        \\
\cite{DBLP:journals/umuai/SymeonidisKZ20} & UMUAI     & 2020 &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        & \cmark &        &        &        &        &        & \cmark &        &        &        &        &        &        & \cmark &        \\
\cite{DBLP:conf/sigir/SongWJZHH21}        & SIGIR     & 2021 & \cmark &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        & \cmark &        &        &        &        &        &        & \cmark &        &        &        &        &        &        \\
\cite{DBLP:conf/kdd/YuY000H21}            & KDD       & 2022 & \cmark &        &        &        & \cmark &        &        &        &        &        &        &        &        &        &        & \cmark & \cmark & \cmark &        &        &        &        &        &        &        &        &        &        & \cmark &        \\
\cite{DBLP:conf/bigdataconf/BaiZWN20}     & ICBD      & 2020 &        &        &        &        &        &        &        &        &        &        &        &        &        & \cmark &        & \cmark & \cmark &        &        &        &        &        &        &        &        &        &        &        &        & \cmark \\
\cite{DBLP:conf/wsdm/GeLGXLZP0GOZ21}      & WSDM      & 2021 &        &        & \cmark &        &        &        &        &        &        &        &        &        &        &        &        & \cmark & \cmark &        &        &        &        &        &        &        & \cmark &        &        &        & \cmark &        \\
\cite{DBLP:journals/corr/abs-2003-10699}  & Inf. Sci. & 2021 &        &        &        &        &        &        &        &        &        &        &        &        &        &        &        & \cmark &        &        &        &        &        &        & \cmark &        &        &        &        &        & \cmark &        \\
\cite{DBLP:journals/tkde/YuXCCHY24}       & TKDE     & 2022 &        &        &        &        &        &        &        &        &        & \cmark & \cmark &        &        &        &        & \cmark & \cmark &        &        &        &        &        &        & \cmark &        &        &        &        &        &        \\ \midrule
                                         &           &      & 17     & 14     & 10     & 9      & 9      & 8      & 7      & 7      & 4      & 4      & 3      & 3      & 3      & 3      & 3      & 40     & 25     & 15     & 13     & 9      & 4      & 4      & 7      & 21     & 13     & 5      & 4      & 3      & 10     & 1     \\
    \bottomrule
\end{tabular}
\end{table*}

==> tables/models.tex <==
\begin{table}[!t]
\centering
\caption{Overview of multimodal features extractors as employed in recent multimodal recommendation systems. We provide details regarding year, domain, and extractor models adopted for each modality.}
\label{tab:extractors}
\begin{adjustbox}{width=\textwidth, center}
\rowcolors{4}{gray!17.5}{white}
\begin{tabular}{lcccccc}
\toprule
\textbf{Papers} & \textbf{Year} & \textbf{Domain} &
\multicolumn{3}{c}{\textbf{Modalities}}  \\
\cmidrule(lr){4-6}
 \multicolumn{ 1}{c}{}  & \multicolumn{ 1}{c}{} & & \multirow{1}{*}{\textcolor{Mahogany}{Visual}} & \multirow{1}{*}{\textcolor{RoyalBlue}{Textual}} & \multirow{1}{*}{\textcolor{OliveGreen}{Audio}}   \\
\midrule                                                                                             
\citet{DBLP:conf/mm/HanWJD17}     & 2017 & Fashion         & Custom                                                                                                        & Custom                                 &                 \\
\citet{DBLP:conf/recsys/OramasNSS17}    &     2017 &  Music        &                                                                                                              & Custom                                 & Custom          \\
\citet{DBLP:conf/ijcai/ZhangWHHG17}    &       2017 &  Social Media      & Custom                                                                                                 & Custom                                 &                  \\
\midrule                                                                                 
\citet{DBLP:conf/kdd/YingHCEHL18}     & 2018    & E-commerce     & VGG16                                                                                                         & Word2Vec                               &                 \\
\citet{DBLP:conf/emnlp/WangNL18}     &     2018   & E-commerce      & AlexNet                                                                                                         & Custom                          &                 \\
\midrule                                                                                    
\citet{DBLP:conf/mm/LiuCSWNK19}      & 2019   & E-commerce      & AlexNet                                                                                                       & PV-DM                                  &                 \\
\citet{DBLP:conf/sigir/ChenCXZ0QZ19}     &    2019   & Fashion       & VGG19                                                                                                         & Custom                          &                 \\
\citet{DBLP:conf/mm/WeiWN0HC19}      &       2019    & Movie, Social Media   & ResNet50                                                                                                      & Sentence2Vec                        & VGGish          \\
\citet{DBLP:journals/tois/ChengCZKK19}    &    2019      & E-commerce, Restaurant    & ResNet152                                                                                                     & LDA                                &                 \\
\citet{DBLP:conf/mm/DongSFJXN19}     &     2019     & Fashion    & VGG16                                                                                                         & Bag-of-word scheme                     &                 \\
\citet{DBLP:conf/kdd/ChenHXGGSLPZZ19}     &  2019      & Fashion      & Inception ResNet V2                                                                                           & TextCNN                                &                 \\
\citet{DBLP:conf/mm/YuSZZJ19}       &      2019    & Fashion    & ResNet50                                                                                                      & CNN, GRU                              &                 \\
\midrule                                                                                          
\citet{DBLP:journals/tkde/CuiWLZW20}      & 2020 & E-commerce, Fashion         & GoogLeNet                                                                                                     & GloVe                                  &                 \\
\citet{DBLP:conf/mm/WeiWN0C20}      &      2020 & Movie, Social Media        &   \texttt{N/A}                                                                                                            &  \texttt{N/A}                                     &  \texttt{N/A}              \\
\citet{DBLP:conf/cikm/SunCZWZZWZ20}      &      2020 &         Movie, Restaurant & ResNet50                                                                                                      & Word2Vec, SIF                         &                 \\
\citet{DBLP:conf/ijcai/Chen020}    &    2020 & E-commerce          & AlexNet                                                                                                       & KimCNN                                 &                 \\
\citet{DBLP:journals/tmm/MinJJ20}      &     2020 &  Restaurant         &  Custom                                                                                                      &                                        &                 \\
\citet{DBLP:conf/ijcnn/Shen0LWC20}     &      2020 & E-commerce, Music        & ResNet50                                                                                                      & Custom                                 &                 \\
\citet{DBLP:conf/aaai/YangDW20}     &      2020 & Fashion        & VGG                                                                                                           & Glove                                  &                 \\
\citet{DBLP:journals/ipm/TaoWWHHC20}      &      2020 & Movie, Social Media         & ResNet50                                                                                                      & Sentence2Vec                        & VGGish          \\
\citet{DBLP:journals/tcss/YangWLLGDW20}     &      2020 & Social Media        & Inception V3, ResNet50                                                                                        & BiLSTM                                 &                 \\
\midrule
\citet{DBLP:journals/tmm/SangXQMLW21}     & 2021 & Social Media       & VGG, C3D                                                                                                       & TextCNN                                &                 \\
\citet{DBLP:conf/mm/LiuYLWTZSM21}      &     2021 & E-commerce, Movie         & Inception-v4                                                                                                  & BERT                                   & VGGish          \\
\citet{DBLP:conf/mm/Zhang00WWW21}    &       2021 & E-commerce       & AlexNet                                                                                                       & Sentence-BERT &                 \\
\citet{DBLP:conf/bigmm/VaswaniAA21}  &       2021 & Music       &                                                                                                               & Sentence-BERT                          & Custom          \\
\citet{DBLP:journals/eswa/LeiHZSZ21}      &      2021 & Restaurant        & Custom                                                                                         & Custom                      & Custom \\
\citet{DBLP:journals/tomccap/WangDJJSN21}     &      2021 & Restaurant        & VGG19                                                                                                         & TextCNN                                &                 \\
\midrule
\citet{DBLP:journals/tmm/ZhanLASDK22}     & 2022 & Fashion         & ResNet50                                                                                                      & Custom             &                 \\
\citet{DBLP:conf/sigir/WuWQZHX22}       &   2022 & News           & Mask RCNN, ResNet50, ViLBERT                                                                               & ViLBERT                                &                 \\
\citet{DBLP:journals/tmm/YiC22}     &       2022 & E-commerce       &  ResNet50                                                                                                    &   Sentence2Vec                                     &                 \\
\citet{DBLP:conf/sigir/Yi0OM22}       &      2022 & Movie, Social Media        &  \texttt{N/A}                                                                                                            &  \texttt{N/A}                                    &  \texttt{N/A}              \\
\citet{DBLP:conf/mir/LiuMSO022}      &      2022 & E-commerce        & CLIP                                                                                                          & \texttt{N/A}          &                 \\
\citet{DBLP:conf/mm/MuZT0T22}       &       2022 & E-commerce       & AlexNet                                                                                               & Sentence-BERT                          &                 \\
\citet{DBLP:conf/mm/ChenWWZS22}     &       2022 & Movie, Social Media       & ResNet50                                                                                                      & Sentence2Vec                           & VGGish          \\
\citet{DBLP:journals/corr/abs-2211-06924}   &      2022 &  E-commerce       & AlexNet                                                                                                      & Sentence-BERT                          &                 \\
\midrule
\citet{DBLP:journals/tmm/WangWYWSN23}     & 2023 & Movie, Social Media         &  ResNet50                                                                                                   &  Sentence2Vec                                      &  VGGish               \\
\citet{DBLP:conf/www/WeiHXZ23}      &      2023 & E-commerce, Restaurant, Social Media        & Custom                                                                                                          & Sentence-BERT                          &                  \\
\citet{DBLP:conf/www/ZhouZLZMWYJ23}     &     2023 & E-commerce         & AlexNet & Sentence-BERT                          &          \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}
